Sparse Representation of 3D Images for Piecewise Dimensionality Reduction with High Quality Reconstruction

Sparse representation of 3D images is considered within the context of data reduction. The goal is to produce high quality approximations of 3D images using fewer elementary components than the number of intensity points in the 3D array. This is achieved by means of a highly redundant dictionary and a dedicated pursuit strategy especially designed for low memory requirements. The benefit of the proposed framework is illustrated in the first instance by demonstrating the gain in dimensionality reduction obtained when approximating true color images as very thin 3D arrays, instead of performing an independent channel by channel approximation. The full power of the approach is further exemplified by producing high quality approximations of hyper-spectral images with a reduction of up to 371 times the number of data points in the representation.

==> table2.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{||r|r|r|r|r||r|r|r|r||}
\hline \hline
I&dB&$\bjp$&$\bsr$&G&dB&$\bjp$&$\bsr$&G \\\hline \hline
1&  45.3&  7.1& 6.6& 8& 40.5 & 4.4 &  4.4&  0 \\ \hline 
2&  43.5&  5.6& 3.5& 38& 40.2&  3.0&  2.2&  29 \\ \hline
3&  45.1&  4.6& 2.5& 46& 42.2&  2.4& 1.6 & 31 \\ \hline 
4&  44.7&  5.5& 4.0& 27& 40.9&  3.1&  2.4&  21 \\ \hline
5&  42.8&  7.5& 5.8& 22& 39.2&  4.6& 4.3 & 8  \\ \hline
6&  44.8&  6.2& 5.0& 19& 40.7&  3.6& 3.2 & 11 \\ \hline
7&  45.3&  5.1& 3.3& 36& 41.9&  2.7& 2.0 & 25 \\ \hline
8&  43.2&  7.7& 6.4& 16& 39.2&  4.7& 4.5 & 5  \\ \hline
9&  45.8&  5.1& 3.9& 25& 41.7&  2.7& 2.0 & 28 \\ \hline
10&  45.3&  5.3& 3.9& 26& 41.4&  2.8& 2.1&  25 \\ \hline
11&  45.4&  6.0& 5.0& 17& 40.9&  3.4& 3.0&  10 \\ \hline
12&  46.1&  5.0& 3.7& 25& 42.2&  2.7& 2.1&  22 \\ \hline
13&  42.9&  8.4& 7.5& 10& 38.7&  5.2& 5.5&  -4 \\ \hline
14&  41.8&  6.8& 4.6& 33& 39.0&  4.1& 3.5&  16 \\ \hline
15&  43.9&  5.2& 3.2& 39& 40.8&  2.8& 2.0&  28 \\ \hline
16&  47.0&  5.3& 4.5& 15& 42.2&  3.0& 2.5&  15 \\ \hline
17&  45.3&  5.4& 4.1& 25& 41.5&  3.0& 2.4&  21 \\ \hline
18&  42.9&  7.0& 5.7& 18& 39.0&  4.1& 3.7&  10 \\ \hline
19&  45.5&  6.0& 5.1& 15& 41.0&  3.4& 2.9&  14 \\ \hline
20&  44.4&  4.5& 3.2& 29& 41.2&  2.4& 2.0&  15\\ \hline
21&  44.6&  6.1& 4.9& 20& 40.5&  3.4& 3.0&  5 \\ \hline
22&  43.0&  6.3& 4.6& 27& 39.5&  3.5& 3.0&  16 \\ \hline
23&  43.9&  4.7& 2.1& 55& 41.3&  2.4& 1.2&  49 \\ \hline
24&  40.0&  6.5& 4.0& 39& 38.0&  3.9& 3.2&  18 \\ \hline \hline
{\bf{mv}}& {\bf{44.3}}&{\bf{6.0}} & {\bf{4.5}}& {\bf{26}}&
{\bf{40.1}}& {\bf{3.4}} & {\bf{2.9}} & {\bf{17}} \\ \hline
{\bf{std}}& {\bf{1.5}}  &{\bf{1.0}} & {\bf{1.3}} & {\bf{11}}& {\bf{1.2}}& {\bf{0.8}}  & {\bf{1.0}} & {\bf{11}}\\ \hline
\end{tabular}
\end{center}
\caption{Comparison of size rate between the JPEG 
file ($\bjp$) and the sparse representation ($\bsr$) 
files for the 
values of PSNR in the $2\mathrm{nd}$ and $6\mathrm{th}$ columns. The average times 
for producing the 4th and 8th columns  are $75\, \mathrm{s}$ and $53\, \mathrm{s}$ 
respectively.}
\label{TABLE2}
%The 6th and 7th are the corresponding gains (c.f \eqref{gain})}
\end{table}

